Errata Note: Discovering Order Dependencies through Order Compatibility

A number of extensions to the classical notion of functional dependencies have been proposed to express and enforce application semantics. One of these extensions is that of order dependencies (ODs), which express rules involving order. The article entitled "Discovering Order Dependencies through Order Compatibility" by Consonni et al., published in the EDBT conference proceedings in March 2019, investigates the OD discovery problem. They claim to prove that their OD discovery algorithm, OCDDISCOVER, is complete, as well as being significantly more efficient in practice than the state-of-the-art. They further claim that the implementation of the existing FASTOD algorithm (ours)-we shared our code base with the authors-which they benchmark against is flawed, as OCDDISCOVER and FASTOD report different sets of ODs over the same data sets. In this rebuttal, we show that their claim of completeness is, in fact, not true. Built upon their incorrect claim, OCDDISCOVER's pruning rules are overly aggressive, and prune parts of the search space that contain legitimate ODs. This is the reason their approach appears to be "faster" in practice. Finally, we show that Consonni et al. misinterpret our set-based canonical form for ODs, leading to an incorrect claim that our FASTOD implementation has an error.

==> ack.tex <==
\section{Acknowledgements} \label{section:ack}
The authors would like to thank Yuliya Lytvyn from University of Toronto for helping us to create the video of the demonstration (Footnote~\ref{foot:yl}).


==> addendum.tex <==
\section{Foundations}\label{sec:foundations}
\subsection{Background}

We use the following notational conventions.

\begin{table}[h]
\caption{Notational conventions.}
\label{table:Notation}
\centering
\begin{normalsize}
\begin{itemize}
    \item \textbf{Relations.}
            \R{R}\ denotes a {\em relation schema} and
            \T{r}\ denotes a specific {\em table} instance.
            Letters from the beginning of the alphabet \A{A}, \A{B}\ and \A{C}\
            denote single \emph{attributes}.
            Additionally, \tup{t}\ and \tup{t}\
            denotes \emph{tuples} and
            \proj{t}{\A{A}}\ denotes
            the value of an attribute \A{A}\ in a tuple \tup{t}.
    \item \textbf{Sets.}
            Letters from the end of the alphabet \set{X}, \set{Y}, and \set{Z}\ denote \emph{sets} of attributes.
            Also, \proj{t}{\set{X}}\ denotes
            the \emph{projection} of a tuple \emph{t} on \set{X}.
            \set{XY}\ is shorthand for \(\set{X}\ \cup \set{Y}\). The empty set is denoted as $\emptySet{}$.

    \item \textbf{Lists}
            \lst{X}, \lst{Y}\ and \lst{Z}\ denote \emph{lists}. The empty list is represented as $\emptyLst{}$.
            List \Lst{\A{A}, \A{B}, \A{C}}\ denotes an explicit list.
            \Lst{\A{A}}[\lst{T}]\
            denotes a list with the \emph{head} \A{A}\
            and the \emph{tail} \lst{T}.
            % (the remaining list when the first element is removed).
            \lst{XY}\ is shorthand for \lst{X}\ concatenate \lst{Y}.
            Set \set{X}\ denotes the {\em set} of elements
            in {\em list} \lst{X}. $\lst{X}'$ denotes any arbitrary permutation of list $\lst{X}$ or set $\set{X}$. Given the set of attributes $\set{X}$, for brevity, we state $\forall i$, $\A{X}_{i}$ to indicate indices $[1, ..., i]$ that have valid ranges ($i \leq |\set{X}|$).
            %Anyplace a set is expected but a list appears,
            % list is {\em cast} to a set;
            %e.g.,
            %\proj{t}{\lst{X}}\ denotes \proj{t}{\set{X}}.
%\line(1,0){220}
\end{itemize}
\end{normalsize}
\end{table}

Next, we provide a summary of the relevant definitions.
%
The operator `\orelOP[\lst{X}]' defines a {\em weak total order} over any set of tuples, where $\lst{X}$ denotes a list of attributes. Unless otherwise specified, numbers are ordered numerically, strings are ordered lexicographically and dates are ordered chronologically.

\begin{definition}\label{definition:operatorle}
Let \lst{X}\ be a list of attributes. For two tuples \tup{t}\ and \tup{s}, $\set{X} \in \R{R}$,
%(over a schema containing the attributes in \lst{X})
\(\tup{t}\orel[\lst{X}]\tup{s}\) if
\begin{itemize}
\item[--]
    \(\lst{X} = \Lst{}\);
    {\em or}
\item[--]
    \(\lst{X} = \Lst{\A{A}}[\lst{T}]\)
    and \(\tup{t}[\A{A}] < \tup{s}[\A{A}]\); or
\item[--]
    \(\lst{X} = \Lst{\A{A}}[\lst{T}]\),
    \(\tup{t}[\A{A}] = \tup{s}[\A{A}]\),
    and
    \(\tup{t}\orel[\lst{T}]\tup{s}\).
\end{itemize}
Let \(\tup{t}\orelStrict[\lst{X}]\tup{s}\) if
    \(\tup{t}\orel[\lst{X}]\tup{s}\) but
    \(\tup{s}\notOrel[\lst{X}]\tup{t}\).
\end{definition}

Next, we define order dependencies~\cite{CSM19}.

\begin{definition}\label{definition:OrderDependency}
Let \lst{X}\ and \lst{Y}\ be lists of attributes, where $\set{X}, \set{Y} \subseteq \R{R}$. \orders{\lst{X}}{\lst{Y}}\ denotes an {\em order dependency} (OD), read as \lst{X}\ {\em orders} \lst{Y}.
%
Table \T{r}\ over $\R{R}$ {\em satisfies} \orders{\lst{X}}{\lst{Y}}\ (\(\T{r} \models \orders{\lst{X}}{\lst{Y}}\))
if, for all \(\tup{t}, \tup{s} \in \T{r}\), \(\tup{t}\orel[\lst{X}]\tup{s}\) implies \(\tup{t}\orel[\lst{Y}]\tup{s}\).
%
\orders{\lst{X}}{\lst{Y}}\ is said to {\em hold} for \R{R}\ (\(\R{R} \models \orders{\lst{X}}{\lst{Y}}\)) if, for each admissible table instance \T{r}\ of \R{R}, table \T{r}\ satisfies \orders{\lst{X}}{\lst{Y}}.
%
\orders{\lst{X}}{\lst{Y}}\ is {\em trivial} if, for all \T{r}, \(\T{r} \models \orders{\lst{X}}{\lst{Y}}\). \orderEquiv{\lst{X}}{\lst{Y}}, read as \lst{X}\ and \lst{Y}\ are {\em order equivalent}, if $\orders{\lst{X}}{\lst{Y}}$ and $\orders{\lst{X}}{\lst{Y}}$.
%(This is written as \(\models \orders{\lst{X}}{\lst{Y}}\).)
\end{definition}

The OD $\orders{\lst{X}}{\lst{Y}}$ means that $\lst{Y}$ values are monotonically non-decreasing with respect to $\lst{X}$ values. Thus, if a list of tuples is ordered by $\lst{X}$, then it is also ordered by $\lst{Y}$, but not necessarily vice versa.

\begin{example}\label{example:taxes}
Consider Table~\ref{table:taxes} in which tax is calculated as a percentage of salary, and tax groups and subgroups are based on salary.  Tax, percentage and group increase with salary.  Furthermore, within the same group, subgroup increases with salary.  Finally, within the same year, bin increases with salary.  Thus, the following ODs hold:
%\begin{enumerate}
    $\orders{ \Lst{ \A{salary} } }{ \Lst{ \A{tax} } }$,
     $\orders{ \Lst{ \A{salary} } }{ \Lst{ \A{percentage} } }$,
    $\orders{ \Lst{ \A{salary} } },
        { \Lst{ \A{group}, \A{subgroup} } }$ and 
    $\orders{ \Lst{ \A{year, salary} } }{ \Lst{ \A{year}, \A{bin} } }$.
%\end{enumerate}
\end{example}

\begin{definition}
    \label{definition:orderCompatible}
Two order specifications \lst{X}\ and \lst{Y}\ are {\em order
compatible}, denoted as \(\lst{X} \sim \lst{Y}\), if
\orderEquiv{\lst{XY}}{\lst{YX}}. ODs in the form of $\simular{\lst{X}}{\lst{Y}}$ are called order compatible dependencies (OCDs)
\end{definition}

The empty list of attributes (i.e., $\emptyLst{}$) is order compatible with {\em any} list of attributes.

There is a strong relationship between ODs and FDs. Any OD implies an FD, modulo lists and sets, however, not vice versa.

\begin{lemma}\label{theorem:relationship}
If $\R{R}$ $\models$ \orders{\lst{X}}{\lst{Y}}\ (OD), then $\R{R}$ $\models$ $\set{X} \rightarrow \set{Y}$ (FD).
\end{lemma}

Also, there exists a correspondence between FDs and ODs.
%that is directly related to the first condition in Theorem~\ref{theorem:orderdependency}.
%
\begin{theorem} \label{theorem:correspondence}
$\R{R}$ $\models$ $\set{X} \rightarrow \set{Y}$ emph{iff} \orders{\lst{X}}{\lst{XY}}, for any list \lst{X}\ over the attributes of \set{X}\ and any list \lst{Y}\ over the attributes of \set{Y}.
\end{theorem}

ODs can be violated in two ways. 

\begin{theorem}\label{theorem:orderdependency}
$\R{R}$ $\models$ \orders{\lst{X}}{\lst{Y}}\ (OD) \emph{iff}
$\R{R}$ $\models$ $\orders{\lst{X}}{\lst{XY}}$ (FD) and $\simular{\lst{X}}{\lst{Y}}$ (OCD).
\end{theorem}

We are now ready to explain the two sources of OD violations: \emph{splits} and \emph{swaps}~\cite{Szl2012}.  An OD $\orders{\lst{X}}{\lst{Y}}$ can be violated in two ways, as per Theorem~\ref{theorem:orderdependency}. 
%
\begin{definition}A \emph{split} wrt an OD $\orders{\lst{X}}{\lst{XY}}$ (i.e., FD) is a pair of tuples \emph{s} and \emph{t} such that $\emph{s}_{\set{X}}$ $=$ $\emph{t}_{\set{X}}$ but
$\emph{s}_{\set{Y}}$ $\not =$ $\emph{t}_{\set{Y}}$.\label{definition:split}
\end{definition}
\begin{definition}A \emph{swap} wrt $\simular{\lst{X}}{\lst{Y}}$ (i.e., with respect to $\orderEquiv{\lst{XY}}{\lst{YX}}$) is a pair of tuples \emph{s} and \emph{t} such that $\emph{s} \prec_{\lst{X}} \emph{t}, \mbox{but}\ \emph{t} \prec_{\lst{Y}} \emph{s}$.
\label{definition:swap}
%(Consequently, \orders{\lst{X}}{\lst{Y}}\ is falsified, too.)
\end{definition}

\begin{example}\label{example:swap} In Table~\ref{table:taxes}, there are three splits with respect to the OD $\orders{ \Lst{ \A{position} } }{ \Lst{ \A{position}, \A{salary} } }$ because \A{position}\ does not functionally determine \A{salary}.  The violating tuple pairs are t1 and t4, t2 and t5, and t3 and t6.
There is a swap with respect to $\simular{ \Lst{ \A{salary} } }{ \Lst{ \A{subgroup} } }$, e.g., over pair of tuples $\tup{t1}$ and $\tup{t2}$.
\end{example}

\subsection{Canonical Forms}

Consonni et al.~\cite{CSM19} uses native list-based canonical form, which is based on decomposing an OD into a FD and an OCD. Recall that based on Theorem~\ref{theorem:orderdependency} ``OD = FD + OCD", as $\orders{\lst{X}}{\lst{Y}}$ \emph{iff} $\orders{\lst{X}}{\lst{XY}}$ (FD) and $\simular{\lst{X}}{\lst{Y}}$ (OCD). The authors exploit this list-based canonical form to guide their discovery algorithm, which leads to factorial complexity in the number of attributes. 

Expressing ODs in a natural way relies on lists of attributes, as in the SQL order-by statement. One might well wonder whether lists are inherently necessary.  We provide a polynomial \emph{mapping} of list-based ODs into \emph{equivalent} set-based canonical ODs~\cite{SGG+17,SGG+18}. The mapping allows us to develop an OD discovery algorithm that traverses a much smaller set-containment lattice rather than the list-containment lattice used in Consonni et al.~\cite{CSM19}.

Two tuples $\tup{t}$ and $\tup{s}$ are \emph{equivalent} over a set of attributes $\set{X}$ if $\proj{t}{\set{X}}$ = $\proj{s}{\set{X}}$. An attribute set $\set{X}$ partitions tuples into \emph{equivalence classes}~\cite{HKP98}. We denote the \emph{equivalence class} of a tuple $\tup{t} \in \T{r}$ over a set $\set{X}$ as follows.

\begin{center}
$\set{E}(\tup{t}_{\set{X}})$, i.e., $\set{E}(\tup{t}_{\set{X}})$ = $\{ \tup{s} \in \T{r}$ $|$ $\proj{s}{\set{X}}$ = $\proj{t}{\set{X}} \}$
\end{center}

A \emph{partition} of $\T{r}$ over $\set{X}$ is the set of equivalence classes, $\Pi_{\set{X}}$ = $\{ \set{E}(\tup{t}_{\set{X}})$ $|$ $\tup{t} \in \T{r} \}$. For instance, in Table~\ref{table:taxes}, $\set{E}(\tup{t1}_{\brac{\A{year}}})$ = $\set{E}(\tup{t2}_{\brac{\A{year}}})$ = $\set{E}(\tup{t3}_{\brac{\A{year}}})$ = $\{ \tup{t1},  \tup{t2}, \tup{t3}\}$ and $\Pi_{\A{year}}$ = $\{ \{ \tup{t1},  \tup{t2}, \tup{t3}\}, \{ \tup{t4},  \tup{t5}, \tup{t6}\} \}$.

We now present a set-based \emph{canonical form} for ODs~\cite{SGG+17,SGG+18}.

\begin{definition}
An attribute $\A{A}$ is a \emph{constant} within each equivalence class over $\set{X}$, denoted as $\set{X}$:$\ordersCst{\emptyLst{}}{\A{A}}$, if $\orders{\lst{X}'}{\lst{X}' \A{A} }$.  Furthermore, two attributes $\A{A}$ and $\A{B}$ are order-compatible (i.e., no swaps) within each equivalence class with respect to $\set{X}$, denoted as $\set{X}$: $\simular{\A{A}}{\A{B}}$, if $\simular{\lst{X}' \A{A}}{\lst{X}' \A{B} }$.  ODs of the form of $\set{X}$:$\ordersCst{\emptyLst{}}{\A{A}}$ and $\set{X}$: $\simular{ \A{A} }{ \A{B} }$ are called \emph{(set-based) canonical} ODs, and the set $\set{X}$ is called a \emph{context}.
\label{def:canonicalODs}
\end{definition}

\begin{example}\label{example:ODs}
In Table~\ref{table:taxes}, $\A{bin}$ is a constant in the context of $\A{position}$ $($$\A{posit}$$)$, written as
    $\brac{\A{position}}$$:$$\ordersCst{\emptyLst{}}{\A{bin}}$.
This is because
    $\set{E}(\tup{t1}_{\brac{\A{position}}})$ $\models$$\ordersCst{\emptyLst{}}{\A{bin}}$,
    $\set{E}(\tup{t2}_{\brac{\A{position}}})$ $\models$$\ordersCst{\emptyLst{}}{\A{bin}}$ and
    $\set{E}(\tup{t3}_{\brac{\A{position}}})$ $\models$$\ordersCst{\emptyLst{}}{\A{bin}}$.
%    
Also, there is no swap between $\A{bin}$ and $\A{salary}$ in the context of $\A{year}$, i.e.,
    $\brac{\A{year}}$$:$ $\simular{\A{bin}}{\A{salary}}$.
This is because
    $\set{E}(\tup{t1}_{\brac{\A{year}}})$ $\models$ $\simular{\A{bin}}{\A{salary}}$ and
    $\set{E}(\tup{t4}_{\brac{\A{year}}})$ $\models$ $\simular{\A{bin}}{\A{salary}}$.
However, the canonical ODs
    $\brac{\A{year}}$$:$ $\simular{\A{bin}}{\A{subgroup}}$
and
    $\brac{\A{position}}$$:$$\ordersCst{\emptyLst{}}{\A{salary}}$
do not hold
as
    $\set{E}(\tup{t1}_{\brac{\A{year}}})$ $\not \models$
        $\simular{\A{bin}}{\A{subgroup}}$ and
    $\set{E}(\tup{t1}_{\brac{\A{position}}})$ $\not \models$$\ordersCst{\emptyLst{}}{\A{salary}}$,
respectively.
\end{example}

Based on Theorem~\ref{thm:canSplitOD} and Theorem ~\ref{thm:canSwapOD} list-based ODs in the form of FDs and OCDs, respectively, can be mapped into equivalent set-based ODs. 

\begin{theorem}
$\R{R}$ $\models$ $\orders{\lst{X}}{\lst{X}\lst{Y}}$ \emph{iff} $\forall \A{A} \in \lst{Y}$, $\R{R}$ $\models$ $\set{X}$$:$$\ordersCst{\emptyLst{}}{\A{A}}$.
\label{thm:canSplitOD}
\end{theorem}

\begin{theorem}
$\R{R}$ $\models$ $\simular{\lst{X}}{\lst{Y}}$ \mbox{\emph{iff}} $\forall i,j$, $\R{R}$ $\models$ $\{ \A{X}_{1}, .., \A{X}_{i-1},$ $\A{Y}_{1}, ..,  \A{Y}_{j-1} \}$$:$ $\simular{\A{X}_{i}}{\A{Y}_{j}}$.
\label{thm:canSwapOD}
\end{theorem}

A list-based OD can be mapped into equivalent set of set-based ODs.

\begin{theorem}
$\R{R}$ $\models$ $\orders{\lst{X}}{\lst{Y}}$ \emph{iff} $\forall \A{A} \in \lst{Y}$, $\R{R}$ $\models$ $\set{X}$$:$$\ordersCst{\emptyLst{}}{\A{A}}$ and $\forall i,j$, $\R{R}$ $\models$ $\{ \A{X}_{1}$, .., $\A{X}_{i-1}$, $\A{Y}_{1}$, ..,  $\A{Y}_{j-1} \}$$:$ $\simular{\A{X}_{i}}{\A{Y}_{j}}$.
%This provides a polynomial mapping of a list-based OD to equivalent set-based canonical ODs.
\label{thm:canonicalODs}
\end{theorem}

The mapping of list-based to set-based ODs is polynomial \emph{(}in the size of the product $|\lst{X}|\times|\lst{Y}|$\emph{)}.

\begin{example}
An OD $\orders{\Lst{\A{A}\A{B}}}{\Lst{\A{C}\A{D}}}$ can be mapped into the following equivalent set of canonical ODs:
    $\brac{\A{A}, \A{B}}$$:$$\ordersCst{\emptyLst{}}{\A{C}}$,
    $\brac{\A{A}, \A{B}}$$:$$\ordersCst{\emptyLst{}}{\A{D}}$,
    $\{\}$: $\simular{\A{A}}{\A{C}}$,
    $\{ \A{A} \}$: $\simular{\A{B}}{\A{C}}$,
    $\{ \A{C} \}$: $\simular{\A{A}}{\A{D}}$,
    $\{ \A{A}, \A{C} \}$: $\simular{\A{B}}{\A{D}}$.
\end{example}

\section{Experimental Analysis}\label{section:evaluation}

We show that experimental analysis in Consonni et al.~\cite{CSM19} to compare their OD discovery algorithm called OCDDISCOVER with our algorithm called FASTOD~\cite{SGG+17,SGG+18} are incorrect. The authors misinterpret the set-base canonical representation introduced in~\cite{SGG+17,SGG+18} by confusing OCDs with ODs. While in~\cite{SGG+17,SGG+18}, we report the number of found FDs and OCDs, the authors in Consonni et al.~\cite{CSM19} falsely report it as the number of FDs and ODs, respectively. This occurs in their Table 6, where for instance, they report the number of 400 ODs and 89,571 FDs found by FASTOD, whereas it should be 400 OCDs and 89,571 FDs, respectively. 

The authors in Consonni et al.~\cite{CSM19} claim that the implementation of FASTOD finds ODs that are not present over the data. As an example they provide an OD $\orders{\Lst{\A{B}}}{\Lst{\A{A},\A{C}}}$ over Table~\ref{table:bug}. However, the FASTOD algorithm finds the following ODs over Table~\ref{table:bug}.

\begin{table}[t]
\begin{center}
\caption{Table showing incompleteness.}
\label{table:sample}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \A{\#} & \A{A} & \A{B} & \A{C} \Tstrut\\
        \hline \hline
        $\tup{t1}$ & 0 &  0 &  1  \Tstrut\\
        \hline
        $\tup{t2}$ & 1 &  1 &  0  \Tstrut\\
        \hline

        \hline
    \end{tabular}
\end{center}
\vskip -0.4cm
\end{table}

\begin{table}[t]
\begin{center}
\caption{Table verifying correctness of implementation.}
\label{table:bug}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \A{\#} & \A{A} & \A{B} & \A{C} & \A{D} \Tstrut\\
        \hline \hline
        $\tup{t1}$ & 1 &  3 &  1 & 1  \Tstrut\\
        \hline
        $\tup{t2}$ & 2 &  3 &  3 & 2  \Tstrut\\
        \hline
         $\tup{t3}$ & 2 &  3 &  2 & 2  \Tstrut\\
        \hline
        $\tup{t4}$ & 2 &  5 &  2 & 2  \Tstrut\\
        \hline
        $\tup{t5}$ & 3 &  1 &  2 & 3  \Tstrut\\
        \hline
        $\tup{t6}$ & 4 &  4 &  4 & 2  \Tstrut\\
        \hline
         $\tup{t7}$ & 4 &  5 &  3 & 2  \Tstrut\\
        \hline
    \end{tabular}
\end{center}
\vskip -0.5cm
\end{table}

\begin{enumerate}
    %\begin{center}
    \item OCD $\{ \A{D} \}$: $\simular{\A{A}}{\A{C}}$
    \item OCD $\{ \A{C} \}$: $\simular{\A{A}}{\A{D}}$
    \item FD $\brac{ \A{A} }$$:$$\orders{\emptyLst{}}{\A{D}}$
    \item OCD $\{ \A{B} \}$: $\simular{\A{A}}{\A{D}}$
    \item OCD $\{ \A{B} \}$: $\simular{\A{C}}{\A{D}}$
    \item OCD $\{ \A{B} \}$: $\simular{\A{A}}{\A{C}}$
    \item FD $\brac{ \A{B}, \A{C} }$$:$$\orders{\emptyLst{}}{\A{D}}$
    \item FD $\brac{ \A{B}, \A{C} }$$:$$\orders{\emptyLst{}}{\A{A}}$
    \item FD $\brac{ \A{A}, \A{B} }$$:$$\orders{\emptyLst{}}{\A{C}}$
    \item OCD $\{ \A{C}, \A{D} \}$: $\simular{\A{A}}{\A{B}}$
    %\end{center}
\end{enumerate}

This shows that authors in Consonni et al.~\cite{CSM19} misinterpret an OCD $\{ \A{B} \}$: $\simular{\A{A}}{\A{C}}$ with and OD $\orders{\Lst{\A{B}}}{\Lst{\A{A},\A{C}}}$. As the consequence, they falsely assert that the reason the number of ODs found by OCDDISCOVER and FASTOD is different, is due to an implementation error in the code that we have provided to the them.%
\footnote{
Note that despite the authors in Consonni et al.~\cite{CSM19} state that they were not able to isolate and resolve the root cause of behaviour of our implementation, they have never contacted us to verify it that we would be happy to help to resolve. The source of FASTOD has been provided by us to the authors through direct communication, due to their request of ``ensuring fairness and reproducability''.
}$^{,}$%
\footnote{
The authors in Consonni et al.~\cite{CSM19} also state that FASTOD considers all columns as if they contain data of type string and their code considers also real and integers numbers. While this comment is minor, we would like to clarify that we sent the authors of Consonni et al.~\cite{CSM19} a file, which allows FASTOD to discover data types including real and integer numbers. 
}
%
However, the real reason is that the algorithm  OCDDISCOVER by Consonni et al.~\cite{CSM19} is incomplete as shown in Section~\ref{section:completness}. 

Thus, the claim in Consonni et al.~\cite{CSM19} that despite a much higher worst-case complexity than FASTOD, it outperforms state-of-art when tested in practice on real datasets is invalid, as the OCDDISCOVER algorithm is not complete. 

%output of Mehdi's code
%[1  SCORE: 27] OCD: { D } : A ~ C
%[2  SCORE: 15] OCD: { C } : A ~ D
%[3  SCORE: 15] FD: {A }: [ ] |--> D
%[4  SCORE: 11] OCD: { C D } : A ~ B
%[5  SCORE: 11] OCD: { B } : A ~ D
%[6  SCORE: 11] OCD: { B } : C ~ D
%[7  SCORE: 11] OCD: { B } : A ~ C
%[8  SCORE: 7] FD: {B, C }: [ ] |--> D
%[9  SCORE: 7] FD: {A, B }: [ ] |--> C
%[10  SCORE: 7] FD: {B, C }: [ ] |--> A

%$\{ \A{A}, \A{C} \}$: $\simular{\A{B}}{\A{D}}$
%$\brac{\A{A}, \A{B}}$$:$$\orders{\emptyLst{}}{\A{C}}$

%they misinterpret the results of FASTOD. 

==> autE.tex <==
\author{Parke Godfrey}
\affiliation{%
  \institution{York University}
  \state{Ontario, Canada} 
}
\email{godfrey@yorku.ca}

\author{Lukasz Golab}
\affiliation{%
  \institution{University of Waterloo}
  \state{Ontario, Canada} 
}
\email{lgolab@uwaterloo.ca}

\author{Mehdi Kargar}
\affiliation{%
  \institution{Ryerson University}
  \state{Ontario, Canada} 
}
\email{kargar@ryerson.ca}

\author{Divesh Srivastava}
\affiliation{%
  \institution{AT\&T Labs-Research}
  \state{New York, United States} 
}
\email{divesh@research.att.com}

\author{Jaroslaw Szlichta}
\affiliation{%
  \institution{Ontario Tech University}
  \state{Ontario, Canada} 
}
\email{jarek@uoit.ca}
